Coarse race data conceals disparities in clinical risk score performance

Healthcare data in the United States often records only a patient's coarse race group: for example, both Indian and Chinese patients are typically coded as "Asian." It is unknown, however, whether this coarse coding conceals meaningful disparities in the performance of clinical risk scores across granular race groups. Here we show that it does. Using data from 418K emergency department visits, we assess clinical risk score performance disparities across 26 granular groups for three outcomes, five risk scores, and four performance metrics. Across outcomes and metrics, we show that the risk scores exhibit significant granular performance disparities within coarse race groups. In fact, variation in performance within coarse groups often *exceeds* the variation between coarse groups. We explore why these disparities arise, finding that outcome rates, feature distributions, and the relationships between features and outcomes all vary significantly across granular groups. Our results suggest that healthcare providers, hospital systems, and machine learning researchers should strive to collect, release, and use granular race data in place of coarse race data, and that existing analyses may significantly underestimate racial disparities in performance.

==> mlhc-camera-ready-template/table_enriched_eci_codes_chi.tex <==
\begin{table}[]
    \centering
    \small
\begin{tabular}{llll}
\toprule
 Coarse Race &    Granular Race &                      ICD Code &  Ratio \\
\midrule
       Asian &      Indian &                Hypothyroidism &   3.14 \\ \cmidrule{2-4} 
        &          Chinese &         Tumor (w/ Metastasis) &   2.06 \\
        &           &        Tumor (w/o Metastasis) &   1.97 \\
        &           &                 Renal Failure &   1.96 \\
        &           &                  Coagulopathy &   1.94 \\
        &           &          Hypertension, Compl. &   1.93 \\ \cmidrule{2-4} 
        & SE Asian  &                   Weight Loss &   2.62 \\
        &  &         Chronic Pulm. Disease &   2.12 \\
        &  &          Hypertension, Compl. &   1.97 \\
        &  &        Tumor (w/o Metastasis) &   1.85 \\
        &  & Fluid Electrolyte Disorders &   1.66 \\ \midrule 
       Black & Black* &                    Drug Abuse &   2.54 \\
        &  &          Rheumatoid Arthritis &   2.20 \\
        &  &                 Alcohol Abuse &   2.11 \\
        &  &                       Obesity &   2.05 \\
        &  &         Chronic Pulm. Disease &   1.98 \\ \midrule 
Hisp./Latino &        Columbian &                Hypothyroidism &   2.01 \\ \cmidrule{2-4} 
 &     Puerto Rican &                    Drug Abuse &   4.14 \\
 &      &         Chronic Pulm. Disease &   2.62 \\
 &      &                     Psychoses &   2.37 \\
 &      &                 Alcohol Abuse &   2.24 \\
 &      &                    Depression &   2.03 \\ \midrule 
       White &       Portuguese &                 Liver Disease &   2.53 \\
        &        &                  Coagulopathy &   2.00 \\
        &        &        Tumor (w/o Metastasis) &   1.84 \\
        &        &            Diabetes, Uncompl. &   1.72 \\ \cmidrule{2-4} 
        &           White* &                    Drug Abuse &   1.59 \\
        &            &                 Alcohol Abuse &   1.32 \\ \cmidrule{2-4} 
        &   Other European &        Tumor (w/o Metastasis) &   1.46 \\
        &    &         Tumor (w/ Metastasis) &   1.45 \\
        &    &                       Obesity &   1.31 \\
        &    &           Cardiac Arrhythmias &   1.21 \\
        &    &        Hypertension, Uncompl. &   1.21 \\ \cmidrule{2-4} 
        &          Russian &          Hypertension, Compl. &   2.82 \\
        &           &            Diabetes, Uncompl. &   2.82 \\
        &           &      Congestive Heart Failure &   2.72 \\
        &           &                 Renal Failure &   2.65 \\
        &           &        Hypertension, Uncompl. &   2.26 \\
\bottomrule
\end{tabular}

\label{tab:enriched_eci_codes}
\caption{\textbf{ECI / Chi} ECI codes that are significantly enriched in a granular race group, as measured by the ratio of the prevalence of an ECI code among patients in a granular race to the prevalence of an ECI code in the remainder of the coarse subgroup. For example, the ECI code for ``Hypothyroidism" is 3.14 times more common among Indian patients compared to patients from other Asian subgroups. All p-values are less than 5e-5, measured using a chi squared test for a difference in proportions. We exclude ECI codes which appear fewer than 10 times in a granular race group for privacy reasons. If a granular race does not appear here, it is because no ECI code is significantly enriched in that group.}
\end{table}

==> mlhc-camera-ready-template/table_enriched_symptoms_chi.tex <==

\begin{table}[]
    \centering
    \tiny

\begin{tabular}{llll}
\toprule
 Coarse Race &       Granular Race &                                                     ICD Code &  Ratio \\
\midrule
       Asian &              Asian* &                 Alcohol abuse with intoxication, unspecified &   2.28 \\ \cmidrule{2-4} 
        &         Indian &                                  Hypothyroidism, unspecified &   2.88 \\
        &         &                          Unspecified acquired hypothyroidism &   2.85 \\ \cmidrule{2-4} 
        &             Chinese & Chronic viral hepatitis B without mention of hepatic coma... &   2.49 \\
        &              &                           Unspecified essential hypertension &   1.59 \\
        &              &                            Acute kidney failure, unspecified &   1.48 \\
        &              &                             Essential (primary) hypertension &   1.45 \\
        &              &                                          Anemia, unspecified &   1.41 \\ \cmidrule{2-4} 
        &              Korean &                                   Alcohol abuse, unspecified &   3.49 \\ \cmidrule{2-4} 
        &    SE Asian  &                             Personal history of tuberculosis &   3.65 \\
        &     &                            Acute kidney failure, unspecified &   1.85 \\ \midrule 
       Black &    Black* &         Other, mixed, or unspecified drug abuse, unspecified &   6.42 \\
        &     &                       Body mass index (BMI) 45.0-49.9, adult &   3.45 \\
        &     &                                               Morbid obesity &   3.44 \\
        &     &               Morbid (severe) obesity due to excess calories &   3.26 \\
        &     & Person boarding or alighting a pedal cycle injured in col... &   3.22 \\ \cmidrule{2-4} 
        &        Cape Verdean & Other viral diseases in the mother, delivered, with or wi... &   4.31 \\
        &         &                              41 weeks gestation of pregnancy &   3.69 \\
        &         &                                          Post-term pregnancy &   3.58 \\
        &         & Post term pregnancy, delivered, with or without mention o... &   3.05 \\
        &         & Second-degree perineal laceration, delivered, with or wit... &   2.57 \\ \cmidrule{2-4} 
        &    Caribbean Island & Nonspecific reaction to tuberculin skin test without acti... &   3.48 \\ \midrule 
Hisp./Latino & Hisp./Latino* & Suicide and self-inflicted injury by cutting and piercing... &   9.53 \\
 &  &      Other and unspecified diseases of the oral soft tissues &   8.26 \\
 &  & Unspecified drug or medicinal substance causing adverse e... &   7.02 \\
 &  &       Acute alcoholic intoxication in alcoholism, continuous &   6.81 \\
 &  &                                             Other acute pain &   6.67 \\ \cmidrule{2-4} 
 &    Central American & Nonspecific reaction to tuberculin skin test without acti... &   5.42 \\ \cmidrule{2-4} 
 &           Dominican & Other specified pregnancy related conditions, first trime... &   2.96 \\
 &            & Abnormality in fetal heart rate and rhythm complicating l... &   2.83 \\
 &            &                                            Single live birth &   2.09 \\
 &            &                             Essential (primary) hypertension &   1.37 \\ \cmidrule{2-4} 
 &        Puerto Rican & Poisoning by heroin, accidental (unintentional), initial ... &  12.27 \\
 &         &                                  Opioid abuse, uncomplicated &   4.46 \\
 &         &           Unspecified viral hepatitis C without hepatic coma &   3.06 \\
 &         &               Nicotine dependence, cigarettes, uncomplicated &   2.47 \\
 &         &                            Unspecified asthma, uncomplicated &   1.96 \\ \midrule 
       White &          Portuguese &                            Spontaneous bacterial peritonitis &   6.17 \\
        &           &                    Hepatic failure, unspecified without coma &   5.17 \\
        &           &                       Other diseases of stomach and duodenum &   4.89 \\
        &           &                    Alcoholic cirrhosis of liver with ascites &   4.81 \\
        &           &                Secondary esophageal varices without bleeding &   4.76 \\ \cmidrule{2-4} 
        &              White* & Driver of heavy transport vehicle injured in collision wi... &   5.77 \\
        &               &                           Unspecified episodic mood disorder &   4.16 \\
        &               &                 Alcohol abuse with intoxication, unspecified &   3.13 \\
        &               &                                                 Homelessness &   2.93 \\
        &               &        Other and unspecified alcohol dependence, unspecified &   2.74 \\ \cmidrule{2-4} 
        &           Brazilian &                                            Acute pharyngitis &   3.47 \\
        &            & Motorcycle driver injured in collision with fixed or stat... &   3.45 \\
        &            &                                            Single live birth &   3.05 \\ \cmidrule{2-4} 
        &      Other European &                  Obstructive sleep apnea (adult) (pediatric) &   1.46 \\
        &       &         Gastro-esophageal reflux disease without esophagitis &   1.31 \\
        &       &                                  Hyperlipidemia, unspecified &   1.30 \\
        &       &                             Essential (primary) hypertension &   1.30 \\
        &       &                      Personal history of nicotine dependence &   1.29 \\ \cmidrule{2-4} 
        &             Russian &    Unspecified hypertensive heart disease with heart failure &   9.06 \\
        &              &                                           Bifascicular block &   6.45 \\
        &              &           Dementia, unspecified, with behavioral disturbance &   6.27 \\
        &              &                             Body Mass Index 27.0-27.9, adult &   5.51 \\
        &              &                              Peripheral vertigo, unspecified &   5.36 \\
\bottomrule
\end{tabular}

\caption{\textbf{ICD / Chi} ICD codes that are significantly enriched in a granular race group, as measured by the ratio of the prevalence of an ICD code among patients in a granular race to the prevalence of an ICD code in the remainder of the coarse subgroup. For example, the ICD code for ``Hypothyroidism" is 2.9 times more common among Indian patients compared to patients from other Asian subgroups. All p-values are less than 2e-7, measured using a chi squared test for a difference in proportions. We exclude ICD codes which appear fewer than 10 times in a granular race group for privacy reasons. If a granular race does not appear here, it is because no ICD code is significantly enriched in that group. \divya{todos:  reorder so that the group with the asterisk appears first. Maybe we highlight ones for which we've found supporting citations?} \nikhil{small nit: just say the words "multiple hypothesis Bonforroni correction" to make obvious that you did this}}
    \label{tab:enriched_icd_codes}

\end{table}

==> mlhc-camera-ready-template/table_permutation_test_risk_score.tex <==
\begin{table}
\centering

\caption{\textbf{Granular variation in the predictive value of the NEWS clinical risk score.} For each metric and coarse group, asterisks denote whether there is significant  \granularvariation\ comparing to a permuted null distribution. `Average' measures the mean \granularvariation\ across the four coarse groups. *$p < 0.05$, **$p < 0.01$, ***$p < 0.001$, \texttt{-} not significant.}

\label{table:news_score_permutation}
\begin{tabular}{l|lcccc}
\toprule
    \textbf{Outcome} & \textbf{Metric} & \textbf{AUPRC} & \textbf{AUROC} &  \textbf{FNR} &  \textbf{FPR} \\
% {} & \textbf{coarse} &       &       &     &      \\
\midrule
\multirow{5}{*}{\textbf{Hospitalization}} & \textbf{Average} &     * &   *** &   * &  *** \\
        & \textbf{Asian} &     - &   *** &   - &    - \\
        & \textbf{Black} &     - &   *** &   - &  *** \\
        & \textbf{White} &     - &   *** &   - &    * \\
        & \textbf{Hispanic/Latino} &     - &   *** &   - &    * \\
\midrule
\multirow{5}{*}{\textbf{Critical}} & \textbf{Average} &     * &     * &   * &  *** \\
        & \textbf{Asian} &     - &     - &   - &    - \\
        & \textbf{Black} &     - &     - &   - &  *** \\
        & \textbf{White} &     - &     * &  ** &   ** \\
        & \textbf{Hispanic/Latino} &     - &     - &   - &    * \\
\midrule
\multirow{5}{*}{\textbf{Revisit}} & \textbf{Average} &     * &    ** &   * &  *** \\
        & \textbf{Asian} &     - &     - &   - &    - \\
        & \textbf{Black} &     - &   *** &   - &  *** \\
        & \textbf{White} &     - &     - &   - &    * \\
        & \textbf{Hispanic/Latino} &     - &     * &   - &    * \\
\bottomrule
\end{tabular}

\end{table}
